Superiorization of Incremental Optimization Algorithms for Statistical Tomographic Image Reconstruction

We propose the superiorization of incremental algorithms for tomographic image reconstruction. The resulting methods follow a better path in its way to finding the optimal solution for the maximum likelihood problem in the sense that they are closer to the Pareto optimal curve than the non-superiorized techniques. A new scaled gradient iteration is proposed and three superiorization schemes are evaluated. Theoretical analysis of the methods as well as computational experiments with both synthetic and real data are provided.

==> inc_iterations.tex <==
\def\xaxisLabels{[]\tiny$0.00$;\tiny$31.75$;\tiny$63.50$;\tiny$95.25$;\tiny$127.00$[]}%
\def\xaxisValues{[]0.00000;0.25000;0.50000;0.75000;1.00000[]}%
\def\yaxisLabels{[]\tiny$-1.46\cdot 10^{11}$;\tiny$-1.45\cdot 10^{11}$;\tiny$-1.45\cdot 10^{11}$[]}%
\def\yaxisValues{[]0.00000;0.50000;1.00000[]}%

